Single-dimensional Contract Design: Efficient Algorithms and Learning

We study a Bayesian contract design problem in which a principal interacts with an unknown agent. We consider the single-parameter uncertainty model introduced by Alon et al. [2021], in which the agent's type is described by a single parameter, i.e., the cost per unit-of-effort. Despite its simplicity, several works have shown that single-dimensional contract design is not necessarily easier than its multi-dimensional counterpart in many respects. Perhaps the most surprising result is the reduction by Castiglioni et al . [2025] from multi- to single-dimensional contract design. However, their reduction preserves only multiplicative approximations, leaving open the question of whether additive approximations are easier to obtain than multiplicative ones. In this paper, we answer this question -- to some extent -- positively. In particular, we provide an additive PTAS for these problems while also ruling out the existence of an additive FPTAS. This, in turn, implies that no reduction from multi- to single-dimensional contracts can preserve additive approximations. Moreover, we show that single-dimensional contract design is fundamentally easier than its multi-dimensional counterpart from a learning perspective. Under mild assumptions, we show that optimal contracts can be learned efficiently, providing results on both regret and sample complexity.

==> src/additivePTAS.tex <==
\section{additive PTAS}

Discretizzare e fare un menu diretto deterministico (epsonenziale nel numero di tipi) e poi usare linearizzazione.

Here, we show that the problem admits an additive PTAS.

Divide the space of types in segments and find an optimal contract/menu $\epsilon$-IC with a constant number of types.

Robustify the solution.



\section{hardness}

\begin{theorem}
	No additive FPTAS.
\end{theorem}

\begin{proof}
	We reduce from set cover.
	%
	Given a set of elements $E$ and a set of sets $\Scal \subset 2^E$, we reduce from the decision problem of determining if there exists a set cover of size $k$, i.e., a set $\Scal^*\subseteq \Scal$ of size $k$ such that 
	$\cup_{S \in \Scal^*} S=E$. This problem is well known to be NP-Hard \cite{feige..}.
	
	We show that if there exists a set cover of size $k$, then principal's utility from the optimal contract is at least $\gamma$ where $\gamma$ will be defined in the following, while if all the set covers have size at least $k+1$ then the utility is at most $\gamma-|E|^{-14}|S|^{-1}$.
	
	\textbf{Construction.}
	%
	Let rename the elements of $E$ as $1,2,\ldots, n$, where $|E|=n$.
	Let $|\mathcal{S}|=m$.
	Moreover, let define  $\rho=n^{-6}$, $\eta=n^{-2}$, $\epsilon=n^{-8}m^{-1}$, and $\ell=n^{-9}m^{-1}$
	%
	%Moreover, when we write $(i,j)=e\in E$, we always assume that $i>j$.
	The instance includes an outcome $\omega_{S}$ with reward $r_{\omega_S}=0$ for each $S \in \Scal$.
	Moreover, it includes an outcome $\omega^*$ with $r_{\omega^*}=0$ and an outcome $\bar \omega$ with $r_{\bar \omega}=0$.
	
	The action available to the agent are the following.
	For each set $S\in \Scal$ and $i\in S$, an action $a_{i,S}$ with $F_{a_{i,S},\omega_S}=\frac{1}{10i}\ell$,  $F_{a_{i,S}, \omega^*}=\frac{1}{5i}\ell$, and $F_{a_{i,S},\bar \omega}=1-\frac{1}{10i}\ell-\frac{1}{5i}\ell$, where we recall that $i\in \mathbb{N}$ is an integer denoting an element.
	The cost of the action is $c_{a_{i,S}}=\frac{1}{20i^2}\ell$. 
	For each set $S$ and each $i\in S$, an action $\bar a_{i,S}$ with $F_{\bar a_{i,S},\omega_S}=\frac{1}{10i}(1-\eta/2)\ell$, $F_{\bar a_{i,S},\bar \omega}=1-\frac{1}{10i}(1-\eta/2)\ell$, and $c_{\bar a_{i,S}}=\frac{1}{20i^2} (1-\eta)\ell$.
	An action $a^*$ with cost $c_{a^*}=1$, $F_{a^*,\omega_S}=\epsilon$ for all $S\in \mathcal{S}$ and $F_{a^*,\omega^*}=1-m\epsilon$.
	
	Finally, the agent's types include a type $\theta=i$ for each $i\in E$, and an additional type $\theta=0$.
	\mat{ricordare di normalizzare i tipi tra 0 e 1se vogliamo.}
	
	The distribution is defined as follows: $\mu_{i}=\frac{1-\rho}{n}$ for each $i \in E$ and $\mu_0=\rho$.
	
	
	
	
	\textbf{if.}
	Suppose that there exists a set cover $\Scal^*$ of size $k$.
	We build a contract with utility at least 
	\[\gamma=	 \frac{1-\rho}{n} \ell \sum_{i} \frac{1}{10i} + \rho (1-m\epsilon) - \rho \epsilon |\Scal^*|  \]
	as follow.
	For each set $S\in \Scal^*$, set
	$p_{\omega_S}=1$.
	Moreover, let $p_{\omega^*}=p_{\bar \omega}=0$ and $p_{\omega_S}=0$ for all $S\notin \Scal^*$.
	
	Then, we compute the best responses for each possible agent's type.
	Consider a type $\theta=i$, $i \in V$.
	Since $\Scal$ is a set cover, there exists a set $S \in \Scal^*$ such that $i \in S$.
	We show that $a_{i,S}$ is a best response for the agent of type $i$.
	For an agent of type $i$, the utility of playing an action $a_{j, S}$ is
	\[
	 \sum_{\omega \in \Omega} F_{ a_{j, S}, \omega } p_\omega - i \cdot c_{a_{j, S}} 
	 \]
	
	
	The agent's utility playing action $a_{i,S}$ is 
	\[ \frac{1}{10i}\ell p_{\omega_{S}} - \frac{1}{20i}\ell=\frac{1}{20i}\ell. \]
	
	We show that the utility playing any other action is not higher.
	The agent utility playing an action $a_{j,S'}$, $S'\in \Scal$, $j \in S'$  is at most 
	\[ \frac{1}{10j}\ell p_{\omega_{S'}} -\frac{i}{20j^2}\ell\le \frac{1}{10j}\ell -\frac{i}{20j^2}\ell\le\frac{1}{20i}\ell. \]
	\mat{trovare modo  elegante per dimostrarlo. foglio martino?}
	
	Playing an action ${\bar a_{j,S'}}$, $S'\in \Scal$, $j \in S'$ , the agent's utility is at most
	\[ \frac{1}{10j} (1-\eta/2)\ell p_{\omega_{S'}}-\frac{i}{20j^2} (1-\eta) \ell\le  \frac{1}{10j} (1-\eta/2)\ell -\frac{i}{20j^2} (1-\eta) \ell \]
	The utility is maximized for $j=i$ getting utility $1/i$.
	Indeed, the maximum is at
	\[ j= i \frac{1-\eta}{1-\eta/2}  \]
	and the agent utility is 
	\[\frac{1}{10i} (1-\eta/2)\ell-\frac{1}{20i} (1-\eta) \ell=\frac{1}{20i}\ell \]	
	\mat{dimostrare ma anche qui ho pochi dubbi.}
	
	Finally, it is easy to see that the agent's utility playing action $a^*$ is negative.
	Hence, the best response of type $\theta=i$ is $a_{i,S}$.\footnote{dire che questa è quella che rompe i pareggi in favore del principal?}
	
	Finally, consider the type $\theta=0$.
	Taking action $a^*$, the agent's utility is
	\[|\Scal^*|\epsilon\ge \epsilon > \ell, \]
	while the utility taking any other action is at most $\ell$.
	
	Hence, the expected principal's utility is
	\[  \frac{1-\rho}{n} \ell \sum_{i} [\frac{1}{5i}- \frac{1}{10i}] + \rho (1-m\epsilon - \epsilon |\Scal^*|)= \frac{1-\rho}{n} \ell \sum_{i} \frac{1}{10i} + \rho (1-m\epsilon - \epsilon |\Scal^*|) =\gamma . \]
	
	\textbf{only if.}
	Suppose that all set covers have size at least $k+1$.
	%
	We show that any contract has utility at most $\gamma-n^{14}m^{-1}$.
	
	Let $p$ be a contract.
	% First, we show that $p_{\omega^*}<\gamma$.
	%Otherwise, we get that the expected utility is at most
	%\begin{align*}
	%	\rho n + (1-n\rho) (1-|E|\epsilon) - (1-n\rho) (1-|E|\epsilon) p_{\omega^{\star}} \ge \rho \sum_{i} (\frac{1}{2}+\frac{1}{10i}) + (1-n\rho) (1-|E|\epsilon) - (1-n\rho)\epsilon |E^*| -\nu		
	%\end{align*}
	%implying
	%\begin{align}
	%	p_{\omega^{\star}} \le \frac{1}{(1-n\rho) (1-|E|\epsilon)} [\rho n + \epsilon |E| + \nu   ]\le 2 [n^{-6}+n^{-8}+n^{-6}] \le 6 n^{-6} 
	%\end{align}
	We split the set of elements $E$ in three sets.
	$E_1\subseteq E$ includes the elements $i$ such that the best response of type $i$ to contract $p$ is $a_{i,S}$, for an $S \in \Scal$.
	%
	$E_2\subseteq E$ includes  the elements $i$ such that the best response of type $i$ is $a_{j,S}$ with $j\neq i$ and $S \in \Scal$.
	%
	Finally, $E_3=E \setminus (E_1\cup E_2)$.
	
	We start analyzing the constraints that the best responses of types $\theta \in E_1$ impose on the contract.
	Consider a type $\theta=i \in E_1$, and let $a_{i,S}$ be their best response. Notice that $i\in S$.
	%
	Then, from the IC constraint with respect to action $\bar a_{i,S}$ it holds
	
	\[p_{\omega_{S}}\frac{1}{10i}\ell + p_{\omega^*}  \frac{1}{5i}\ell- \frac{1}{20i}\ell \ge  p_{\omega_{S}}\frac{1}{10i} (1-\eta/2)\ell - \frac{1}{20i} (1-\eta) \ell \]
	implying
	\[p_{\omega_{S}}\ge 1-4  p_{\omega^*}/\eta.\]
	
	Now, consider an agent's type $\theta=i\in E_2$, and let $a_{j,S}$, $j \neq i$ be the action played by the agent. 
	Notice that $j \in S$. Then, the IC constraint with respect to action $\bar a_{j,S}$ implies
	\[ p_{\omega_{S}} \frac{1}{10j} \ell + \frac{1}{5j}p_{\omega^*}\ell- \frac{i}{20j^2}\ell \ge p_{\omega_{S}} \frac{1}{10j} (1-\eta/2) \ell- \frac{i}{20j^2} (1-\eta) \ell \]
	and
	%\[ p_{\omega_{S}} \frac{\eta}{20j} \ge  \frac{i\eta}{20j^2} - \frac{1}{5j} p_{\omega^*} \]
	%and
	\[ p_{\omega_{S}} \ge \frac{i}{j}- p_{\omega^*} \frac{4}{\eta}. \]
	
	Hence, the principal's expected utility when the realized type is a $\theta=i \in E_2$ is at most:
	\[ \frac{1}{5j} (1-p_{\omega_{S}}) - \frac{i}{10j^2} +  \frac{1}{10j} p_{\omega^*} \frac{4}{\eta}\le \frac{1}{5j} - \frac{i}{10j^2} +  \frac{1}{10j} p_{\omega^*} \frac{4}{\eta}
	\le \frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*}  \]
	\mat{da dimostrare, ho checkato su wolfram}
	
	Finally, consider the set of agent types $\theta=i\in E_3$. These agent's types play an action $\bar a_{j,S}$, $j\in E$, $S\in \Scal$ or action $a^*$, or \mat{or void action (aggiungere al modello)}. It is easy to see that the principal's utility is at most $0$ for all these possible actions. 
	
	Finally, type $\theta=0$ plays action $a^*$ otherwise the utility is clearly below $\gamma-n^{14}m^{-1}$.
	
	
	
	Let $\bar \Scal$ be the sets $S$ such that $p_{\omega_S}\ge 1- 4 p_{\omega^*}$.
	Then, the principal's utility is at most 
	\[ \frac{1-\rho}{n} \ell \left[\sum_{i \in E_1}( \frac{1}{5i} (1-p_{\omega^{*}}) - \frac{1}{10i}( 1-4p_{\omega^*}/\eta))  + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*})\right] + \rho (1-m\epsilon) (1-p_{\omega^*}) - \rho \epsilon |\bar\Scal|(1-4p_{\omega^*}/\eta)\]
	\[\le \frac{1-\rho}{n} \ell \left[\sum_{i \in E_1}( \frac{1}{5i}  - \frac{1}{10i}( 1-4p_{\omega^*}/\eta))  + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*})\right] + \rho (1-m\epsilon) (1-p_{\omega^*}) - \rho \epsilon |\bar\Scal|(1-4p_{\omega^*}/\eta)   \]
	
	
	Then, since
	\[ \frac{1-\rho}{n} \ell  n \frac{2}{5} \frac{1}{\eta} - \rho (1-m\epsilon) + 4 \rho \epsilon m \frac{1}{\eta} \le  \ell/\eta -\rho/2 + 4 \rho \epsilon m/\eta=n^{-7}m^{-1} - n^{-6}/2 + 4 n^{-12}<0 \]
	for $n$ large enough, it is the case that
	
	\[\arg \max_{p_{\omega^*}}  \frac{1-\rho}{n} \ell [\sum_{i \in V^*}( \frac{1}{5i}  - \frac{1}{10i}( 1-4p_{\omega^*}/\eta))  + \sum_{i \notin V^*} (\frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*})] + \rho (1-m\epsilon) (1-p_{\omega^*}) - \rho \epsilon |\bar\Scal|(1-4p_{\omega^*}/\eta)= 0,\]
	
	Hence, setting $p_{\omega^*}=0$ the principal's utility is at most
	\begin{align}
		&\frac{1-\rho}{n} \ell \left[\sum_{i \in E_1}( \frac{1}{5i}  - \frac{1}{10i})  + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}) \right] + \rho (1-m\epsilon) - \rho \epsilon |\bar\Scal|\\
		&=\frac{1-\rho}{n} \ell \left[\sum_{i \in E_1} \frac{1}{10i} + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}) \right] + \rho (1-m\epsilon) - \rho \epsilon |\bar\Scal|\\
		& \le \frac{1-\rho}{n} \ell \sum_{i \in E} \frac{1}{10i}    + \rho (1-m\epsilon) - \rho \epsilon (|\bar\Scal|+ |E\setminus E_1|) 
	\end{align}
	where the last inequality follows since 
	\[\frac{1-\rho}{n} \ell \frac{1}{40n^3}\ge n^{-13} m^{-1}/80 \ge n^{-14} m^{-1}  = \rho \epsilon. \]
	for $n$ large enough.
	
	Let define the function $s:E\rightarrow\Scal$ that assign to each element $i \in E$ a set $S \in \Scal$ such that $i\in S$.
	Now, notice that there exists a set cover of size $|\bar\Scal|+ |E\setminus E_1|$ taking the set $S=\bar\Scal\cup (\cup_{v \in V\setminus V^*} s(v))$. Indeed, all the elements in $E_1$ are covered by a set in $\Scal$ by definition, while $\cup_{E \in E \setminus E_1} s(v)$ clearly covers all the elements not in $E_1$.
	
	Thus,the principal's utility is at most
	\[ \frac{1-\rho}{n} \ell \sum_{i \in V} \frac{1}{10i}    + \rho (1-m\epsilon) - \rho \epsilon (k+1)\le \gamma - \rho \epsilon= \gamma- n^{-14} m^{-1}, \]
	concluding the proof.
	
	
	
	
	
\end{proof}

\section{martino version}

\section{additive PTAS}


Discretizzare e fare un menu diretto deterministico (epsonenziale nel numero di tipi) e poi usare linearizzazione.


Here, we show that the problem admits an additive PTAS. The algorithm works as follows

For any $\epsilon>0$ consider the set $\tilde\Theta_\epsilon=\{k\epsilon\}_{k=0}^{\lfloor 1/\epsilon\rfloor}$ and compute the probability of each type $\theta \in \tilde\Theta_\epsilon$ as $\tilde \mu_{\theta}:=\int_{\theta-\epsilon/2}^{\theta+\epsilon/2}\mu_\theta d\theta$ for all $\theta\in \tilde\Theta_\epsilon$.\ma{va approssimato forse o fare assunzioni su come mi viene data $\mu_\theta$}. \mat{la cosa più sensata mi pare avere un oracolo che di calcola l'intergrale dato l'intervallo}. Also consider the discrete set of costs $\tilde c_{\theta, a}:=\theta\cdot c_a$ for each $\theta\in\tilde \Theta_\epsilon$. Now consider the bayesian contract design problem defined by the set of types $\tilde \Theta_{\epsilon}$ with distribution $\{\tilde \mu_{\theta}\}_{\theta\in\tilde\Theta_\epsilon}$, costs $\{\tilde c_{a,\theta}\}_{\theta\in\tilde\Theta_\epsilon,a\in A}$, the set of outcomes, outcome distribution and rewards of the principal are left unchanged. \citet[Theorem~8]{castiglioni2022bayesian} gives an algorithm with running time $\poly(n^{1/\epsilon}, m)$ that finds the optimal contract $\tilde p$.

\begin{lemma}
		
\end{lemma}

\begin{lemma}
	A contract $p$ is such that for every $\tilde \theta\in\left[\theta-\frac{\epsilon}{2},\theta+\frac{\epsilon}{2}\right]$ we have that 
	\[
	\sum_{\omega\in\Omega} F_{b^{ \theta}(p),\omega}p_\omega-{\tilde \theta c_{b^{ \theta}(p)}} \ge 	\sum_{\omega\in\Omega} F_{a,\omega}p_\omega-{\tilde \theta c_a }-O(\epsilon)\quad\forall a\in A.
	\]
\end{lemma}

\begin{proof}
	\begin{align}
		\sum_{\omega\in\Omega} F_{b^{ \theta}(p),\omega}p_\omega-{ \theta c_{b^{ \theta}(p)}} &\ge \sum_{\omega\in\Omega} F_{a,\omega}p_\omega-{ \theta c_{a}} \tag{definition of $b^\theta(p)$}\\
		&=\sum_{\omega\in\Omega} F_{a,\omega}p_\omega-{ \tilde\theta c_{a}} +(\tilde\theta-\theta)c_{a}\\
		&\ge \sum_{\omega\in\Omega} F_{a,\omega}p_\omega-{ \tilde\theta c_{a}} -\epsilon/2.
	\end{align}
\end{proof}










\section{hardness}


\begin{theorem}
	No additive FPTAS.
\end{theorem}


\begin{proof}
	We reduce from set cover.
	%
	Given a set of elements $E$ and a set of sets $\Scal \subset 2^E$, we reduce from the decision problem of determining if there exists a set cover of size $k$, i.e., a set $\Scal^*\subseteq \Scal$ of size $k$ such that 
	$\cup_{S \in \Scal^*} S=E$. This problem is well known to be NP-Hard \cite{feige..}.
	
	We show that if there exists a set cover of size $k$, then principal's utility from the optimal contract is at least $\gamma$ where $\gamma$ will be defined in the following, while if all the set covers have size at least $k+1$ then the utility is at most $\gamma-|E|^{-14}|S|^{-1}$.

%	\textbf{Construction.}
%	%
%	Let rename the elements of $E$ as $1,2,\ldots, n$, where $|E|=n$.
%	Let $|\mathcal{S}|=m$.
%	Moreover, let define  $\rho=n^{-6}$, $\eta=n^{-2}$, $\epsilon=n^{-8}m^{-1}$, and $\ell=n^{-9}m^{-1}$
%	%
%	%Moreover, when we write $(i,j)=e\in E$, we always assume that $i>j$.
%	The instance includes an outcome $\omega_{S}$ with reward $r_{\omega_S}=0$ for each $S \in \Scal$.
%	Moreover, it includes an outcome $\omega^*$ with $r_{\omega^*}=0$ and an outcome $\bar \omega$ with $r_{\bar \omega}=0$. \ma{reward sono tutti zero. tbc}
%	
%	The action available to the agent are the following. \ma{$\mu$ non è definito}
%	For each set $S\in \Scal$ and $i\in S$, an action $a_{i,S}$ with $F_{a_{i,S},\omega_S}=\frac{1}{10i}\mu$,  $F_{a_{i,S}, \omega^*}=\frac{1}{5i}\mu$, and $F_{a_{i,S},\bar \omega}=1-\frac{1}{10i}\mu-\frac{1}{5i}\mu$, where we recall that $i\in \mathbb{N}$ is an integer denoting an element.
%	The cost of the action is $c_{a_{i,S}}=\frac{1}{20i^2}\mu$. 
%	For each set $S$ and each $i\in S$, an action $\bar a_{i,S}$ with $F_{\bar a_{i,S},\omega_S}=\frac{1}{10i}(1-\eta/2)\mu$, $F_{\bar a_{i,S},\bar \omega}=1-\frac{1}{10i}(1-\eta/2)\mu$, and $c_{\bar a_{i,S}}=\frac{1}{20i^2} (1-\eta)\mu$.
%	An action $a^*$ with cost $c_{a^*}=1$, $F_{a^*,\omega_S}=\epsilon$ for all $S\in \mathcal{S}$ and $F_{a^*,\omega^*}=1-m\epsilon$.
%	
%	
%	Finally, the agent's types include a type $\theta=i$ for each $i\in E$, and an additional type $\theta=0$.
%	\mat{ricordare di normalizzare i tipi se vogliamo.}
%	
%	The distribution is defined as follows: $\mu_{i}=\frac{1-\rho}{n}$ for each $i \in E$ and $\mu_0=\rho$.
	
	\paragraph{Construction}
	\ma{new construction}
	We identify $E$ with the set $\{1,2,\ldots, n\}$, where $|E|=n$, moreover let $m=|\mathcal{S}|$.
	For ease of presentation, we define  $\rho=n^{-6}$, $\eta=n^{-2}$, $\epsilon=n^{-8}m^{-1}$, and $\ell=n^{-9}m^{-1}$ \ma{$=\mu$?}. \mat{corretto ma dovrei aver rimosso tutti i mu... forse sono rimasti qui ma non sopra.}
	\begin{itemize}
		%
		\item Outcomes
		\begin{itemize}
		\item For each $S \in \Scal$ there is an outcome $\omega_{S}$ 
		%
		\item We define two additional outcomes $\omega^*$ and $\bar \omega$,
		\end{itemize}
		
		\item Rewards
		\begin{itemize}
		\item  For each $S \in \Scal$, reward $r_{\omega_S}=0$. 
		\item $r_{\omega^*}=1$ and $r_{\bar \omega}=0$. 
		\end{itemize}
		
		\item Actions
		\begin{itemize}
			\item For each set $S\in \Scal$ and $i\in S$, we define an action $a_{i,S}$
			\item Moreover, for each set $S\in\Scal$ and each $i\in S$, an action $\bar a_{i,S}$
			\item Additional action $a^*$
			\item $a_0$
		\end{itemize}
		
		\item Action's cost
		\begin{itemize}
			\item $c_{a_{i, S}}=\frac{1}{20 i^2}\mu$ for each $S\in\Scal$ and $i\in S$
			\item $c_{\bar a_{i, S}}=\frac{1}{20 i^2}\mu(1-\eta)$ for each $S\in\Scal$ and $i\in S$
			\item $c_{a^*}=1$
			\item $c_{a_0}=0$
		\end{itemize}
		
		\item Outcome distribution
		\begin{itemize}
		\item For each set $S\in \Scal$ and $i\in S$, $F_{a_{i,S},\omega_S}=\frac{1}{10i}\mu$,  $F_{a_{i,S}, \omega^*}=\frac{1}{5i}\mu$, and $F_{a_{i,S},\bar \omega}=1-\frac{1}{10i}\mu-\frac{1}{5i}\mu$.
		\item \ma{add that $F_{a_{i,S},\omega_{S'}}=0$ for $S\neq S'$?} \mat{dato per scontato ma si puo aggiungere}
		\item For each set $S\in\Scal$ and each $i\in S$, $F_{\bar a_{i,S},\omega_S}=\frac{1}{10i}(1-\frac\eta2)\mu$, $F_{\bar a_{i,S},\bar \omega}=1-\frac{1}{10i}(1-\frac\eta2)\mu$, and $c_{\bar a_{i,S}}=\frac{1}{20i^2} (1-\eta)\mu$.
		\item $F_{a^*,\omega_S}=\epsilon$ for all $S\in\Scal$ and $F_{a^*,\omega^*}=1-m\epsilon$.
		\item $F_{a_0, \bar\omega}=1$
		\end{itemize}
		
		\item Types \mat{ricordare di normalizzare i tipi se vogliamo.}
		\begin{itemize}
			\item The agent's types include a type $\theta=i$ for each $i\in E$, and an additional type $\theta=0$. 
		\end{itemize}
		
		\item Type distribution
		\begin{itemize}
			\item The distribution is defined as follows: $\mu_{i}=\frac{1-\rho}{n}$ for each $i \in E$ and $\mu_0=\rho$.
		\end{itemize}

\mat{in generale credo si possa sostituire 5 10 20 con 1 2 4}
		
%		\item The set of actions available to the agent are the following. \ma{$\mu$ non è definito}
%		For each set $S\in \Scal$ and $i\in S$, we define an action $a_{i,S}$ with $F_{a_{i,S},\omega_S}=\frac{1}{10i}\mu$,  $F_{a_{i,S}, \omega^*}=\frac{1}{5i}\mu$, and $F_{a_{i,S},\bar \omega}=1-\frac{1}{10i}\mu-\frac{1}{5i}\mu$.
%		%
%		
%		\item For each set $S\in\Scal$ and $i\in S$, the cost of action $a_{i,S}$ is $c_{a_{i,S}}=\frac{1}{20i^2}\mu$.
%		
%		\item Moreover, for each set $S\in\Scal$ and each $i\in S$, an action $\bar a_{i,S}$ with $F_{\bar a_{i,S},\omega_S}=\frac{1}{10i}(1-\frac\eta2)\mu$, $F_{\bar a_{i,S},\bar \omega}=1-\frac{1}{10i}(1-\frac\eta2)\mu$, and $c_{\bar a_{i,S}}=\frac{1}{20i^2} (1-\eta)\mu$.
%		
%		\item An action $a^*$ with cost $c_{a^*}=1$, $F_{a^*,\omega_S}=\epsilon$ for all $S\in \mathcal{S}$ and $F_{a^*,\omega^*}=1-m\epsilon$.
%		\item The agent's types include a type $\theta=i$ for each $i\in E$, and an additional type $\theta=0$. 	\mat{ricordare di normalizzare i tipi se vogliamo.}
%		\item The distribution is defined as follows: $\mu_{i}=\frac{1-\rho}{n}$ for each $i \in E$ and $\mu_0=\rho$.
	\end{itemize}
	
	
	
	
	
	\textbf{if.}
	Suppose that there exists a set cover $\Scal^*$ of size less then $k$.
	We build a contract with utility at least 
	\[\gamma=	 \frac{1-\rho}{n} \ell \sum_{i} \frac{1}{10i} + \rho (1-m\epsilon) - \rho \epsilon |\Scal^*|  \]
	as follow.
	For each set $S\in \Scal^*$, set
	$p_{\omega_S}=1$.
	Moreover, let $p_{\omega^*}=p_{\bar \omega}=0$ and $p_{\omega_S}=0$ for all $S\notin \Scal^*$.
	
	Then, we compute the best responses for each possible agent's type.
	
	For an agent of type $i\ge 1$, the utility of playing an action $a_{j, S}$ (for $j\in S$ and $S\in\Scal$) is
	
	\begin{align}
		\sum_{\omega \in \Omega} F_{ a_{j, S}, \omega } p_\omega - i \cdot c_{a_{j, S}} &= \sum_{S'\in\Scal^*} F_{ a_{j, S}, {\omega_{S'}} } p_{\omega_{S'}} - i \cdot c_{a_{j, S}}\\
		&=\sum_{S'\in\Scal^*} F_{ a_{j, S}, {\omega_{S'}} }- i \cdot c_{a_{j, S}}\\
		&=\sum_{S'\in\Scal^*} F_{ a_{j, S}, {\omega_{S'}} }-i \frac{1}{20 j^2}\mu
	\end{align}
	
	If $S\notin \Scal^*$ then the utility of playing $a_{j, S}$ is negative (since $F_{a_{j,S},\omega_{S'}}\neq 0$ if and only if $S=S'$), thus we can assume that $S\in \Scal^*$. Then, continuing from the above, the following holds
	
	\begin{align}
		\sum_{\omega \in \Omega} F_{ a_{j, S}, \omega } p_\omega - i \cdot c_{a_{j, S}} &=\sum_{S'\in\Scal^*} \mathbb{I}(S'=S)\frac{1}{10j}\mu- i\frac{1}{20 j^2}\mu\\
		&=\frac{1}{10j}\mu(1- \frac{i}{2j})
	\end{align}
	
	Now we state that $a_{j, S} = a_{i, S}$ (since $\Scal^*$ is a set cover we know that, for each type $i$, there is a set $S\in \Scal^*$ such that $i\in S$) is the action that maximizes $\frac{1}{10j}\mu(1- \frac{i}{2j})$. This is easily proven by observing that the function $j\mapsto \frac{1}{j}(1-\frac{i}{2j})$ is increasing for $j\le i$ and decreasing for $j\ge i$, thus the maximum incurs at $j=i$ and has utility $\frac{1}{20i}\mu$.
	
	When considering an agent of type $i$, and an action $\bar a_{j, S}$ (for $j\in S$ and $S\in\Scal$), similarly to the case above, we can consider only the case in which $S\in\Scal^*$. Thus we have that the utility of an agent of type $i$, that plays  an action $\bar a_{j, S}$ with $S\in\Scal^*$ is:
	\begin{align}
		\sum_{\omega \in \Omega} F_{ \bar a_{j, S}, \omega } p_\omega - i \cdot c_{\bar a_{j, S}} &= \sum_{S'\in\Scal^*} F_{ \bar a_{j, S}, {\omega_{S'}} }  - i \cdot c_{\bar a_{j, S}}\\
		&=\sum_{S'\in\Scal^*} F_{ \bar a_{j, S}, {\omega_{S'}} }  -i\frac{1}{20j^2}\mu(1-\eta) \\
		&=\frac{1}{10j}(1-\frac\eta2)\mu-i\frac{1}{20j^2}\mu(1-\eta) \\
		&=\frac{1}{10j}\mu\left(1-\frac{\eta}{2}-\frac{i}{2j}(1-\eta)\right).
 	\end{align}

	The we can observe that $j\mapsto \frac{1}{j}\left(1-\frac{\eta}{2}-\frac{i}{2j}(1-\eta)\right)$ is decreasing for $j\le 2i\frac{1-\rho}{2-\rho}$ and increasing otherwise. Since $2i\frac{1-\rho}{2-\rho}\in[i-1, i]$ we only need to compare the utility of $\bar a_{i, S}$ and $\bar a_{i-1, S}$.
	
	Simple calculations shows that the value of action $\bar a_{i-1, S}$ is $\frac{1}{10(i-1)^2}\mu\left[\frac{\eta}{2}(i+1)-1\right]$, while the value of action $\bar a_{i, S}$ is $\frac{1}{20i}\mu$. Straightforward calculations shows that if $\eta\in[0,2(\sqrt{2}-1))$ then $\frac{1}{10(i-1)^2}\mu\left[\frac{\eta}{2}(i+1)-1\right]<\frac{1}{20i}\mu$ and thus $\bar a_{i, S}$ is optimal among all actions $\{\bar a_{i, S}\}_{i, S}$ and gives utility of $\frac{1}{20i}\mu$. However, break ties in favor of the principal, the action $a_{i, S}$ is preferred over action $\bar a_{i, S}$.
	
	
	Indeed the value for the principal of an agent of type $i\ge 0$ playing $a_{i,S}$ (with $S\in \Scal^*$ and $i\in S$) is
	\begin{align}
		\sum_{\omega} F_{a_{i,S},\omega}(r_\omega-p_\omega)&=F_{a_{i,S},\omega^*}r_{\omega^*}-F_{a_{i,S},\omega_S}p_{\omega_S}\\
		&=\frac{1}{5i}\mu-\frac{1}{10i}\mu\\
		&=\frac{1}{5i}\mu
	\end{align}
	while the principal's value when playing $\bar a_{i, S}$ is negative, as the only outcome reachable from playing $\bar a_{i, S}$ are $\omega_S$ and $\bar \omega$ which both have reward of zero.
	
	Now consider that an agent of type $i\ge 1$ plays the action $a^*$. The perceived utility will be
	\begin{align}
		\sum_{\omega\in \Omega} F_{a^*,\omega}p_\omega - i\cdot c_{a^*} & = \sum_{S\in \Scal} F_{a^*,\omega_S} - i\\
		&=\epsilon m - i\\
		&\le 0
	\end{align}
	and thus for each type $i$, the action played would be any action $a_{i,S}$ with $S\in\Scal^*$ and $i\in S$.
	
	Now we have to consider the action played by a type $i=0$. Clearly, an agent of this type wont pay any cost for playing actions. The utility of playing $a^*$ would be at least $m\epsilon$ which is greater then $\mu$. On the other hand the value of playing action $a_{i, S}$ and $\bar a_{i,S}$ (with $i\in S$) would be $\frac{1}{10i}\mu$ and $\frac{1}{10i}\mu(1-\eta/2)$ which are both strictly less then $\mu$. Thus an agent of type $i=0$ will be playing action $a^*$.
	
	Now that we computed the action played by each type we can compute the principal' utility of such contract.
	\begin{align}
		&\sum_{i\ge 1} \mu_i \sum_{\omega\in\Omega}F_{a_{i, S},\omega}(r_\omega-p_\omega) + \mu_0 \sum_{\omega\in\Omega }F_{a^*,\omega}(r_\omega - p_\omega)\\
		&=\sum_{i\ge 1} \frac{1-\rho}{n} \left[F_{a_{i,S},\omega_S}(r_{\omega_S}-p_{\omega_s})+F_{a_{i,S},\omega^*}(r_{\omega^*}-p_{\omega^*})\right]
		 \\
		 &+ \rho(F_{a^*,\omega^*}(r_{\omega^*}-p_{\omega^*})+\sum_{S\in\Scal}F_{a^*,\omega_S}(r_{\omega_S}-p_{\omega_S}))\\
		 &=\frac{1-\rho}{n}\sum_{i\ge 1}\left[\frac{1}{10i}\mu(0-1)+\frac{1}{5i}\mu(1-0)\right]+\rho((1-m\epsilon)(1-0)+|\Scal^*|\epsilon(0-1))\\
		&=\frac{1-\rho}{n} \sum_{i\ge 1} \frac{1}{10i}+\rho(1-m\epsilon-\epsilon|\Scal^*|)=\gamma\\
		&=\frac{1-\rho}{n} \sum_{i\ge 1}\frac{1}{10i}+\rho(1-m\epsilon-\epsilon k):=\gamma
	\end{align}
	
%	\ma{OLD}
%	Consider a type $\theta=i$, $i \in S$.
%	Since $\Scal$ is a set cover, there exists a set $S \in \Scal^*$ such that $i \in S$.
%	We show that $a_{i,S}$ is a best response for the agent of type $i$.
%	The agent's utility playing action $a_{i,S}$ is 
%	\[ \frac{1}{10i}\ell p_{\omega_{S}} - \frac{1}{20i}\ell=\frac{1}{20i}\ell. \]
%	
%	We show that the utility playing any other action is not higher.
%	The agent utility playing an action $a_{j,S'}$, $S'\in \Scal$, $j \in S'$  is at most 
%	\[ \frac{1}{10j}\ell p_{\omega_{S'}} -\frac{i}{20j^2}\ell\le \frac{1}{10j}\ell -\frac{i}{20j^2}\ell\le\frac{1}{20i}\ell. \]
%	\mat{trovare modo  elegante per dimostrarlo. foglio martino?}
%	
%	Playing an action ${\bar a_{j,S'}}$, $S'\in \Scal$, $j \in S'$ , the agent's utility is at most
%	\[ \frac{1}{10j} (1-\eta/2)\ell p_{\omega_{S'}}-\frac{i}{20j^2} (1-\eta) \ell\le  \frac{1}{10j} (1-\eta/2)\ell -\frac{i}{20j^2} (1-\eta) \ell \]
%	The utility is maximized for $j=i$ getting utility $1/i$.
%	Indeed, the maximum is at
%	\[ j= i \frac{1-\eta}{1-\eta/2}  \]
%	and the agent utility is 
%	\[\frac{1}{10i} (1-\eta/2)\ell-\frac{1}{20i} (1-\eta) \ell=\frac{1}{20i}\ell \]	
%	\mat{dimostrare ma anche qui ho pochi dubbi.}
%	
%	Finally, it is easy to see that the agent's utility playing action $a^*$ is negative.
%	Hence, the best response of type $\theta=i$ is $a_{i,S}$.\footnote{dire che questa è quella che rompe i pareggi in favore del principal?}
%	
%	Finally, consider the type $\theta=0$.
%	Taking action $a^*$, the agent's utility is
%	\[|\Scal^*|\epsilon\ge \epsilon > \ell, \]
%	while the utility taking any other action is at most $\ell$.
%	
%	Hence, the expected principal's utility is
%	\[  \frac{1-\rho}{n} \ell \sum_{i} [\frac{1}{5i}- \frac{1}{10i}] + \rho (1-m\epsilon - \epsilon |\Scal^*|)= \frac{1-\rho}{n} \ell \sum_{i} \frac{1}{10i} + \rho (1-m\epsilon - \epsilon |\Scal^*|) =\gamma . \]
%	
	\textbf{only if.}
	Suppose that all set covers have size at least $k+1$.
	%
	We show that any contract has utility at most $\gamma-n^{14}m^{-1}$.
	
	Let $p\in\Reals^{|\Omega|}_{\ge 0}$ be a contract.
	% First, we show that $p_{\omega^*}<\gamma$.
	%Otherwise, we get that the expected utility is at most
	%\begin{align*}
	%	\rho n + (1-n\rho) (1-|E|\epsilon) - (1-n\rho) (1-|E|\epsilon) p_{\omega^{\star}} \ge \rho \sum_{i} (\frac{1}{2}+\frac{1}{10i}) + (1-n\rho) (1-|E|\epsilon) - (1-n\rho)\epsilon |E^*| -\nu		
	%\end{align*}
	%implying
	%\begin{align}
	%	p_{\omega^{\star}} \le \frac{1}{(1-n\rho) (1-|E|\epsilon)} [\rho n + \epsilon |E| + \nu   ]\le 2 [n^{-6}+n^{-8}+n^{-6}] \le 6 n^{-6} 
	%\end{align}
	We partition the set of elements $E$ in three sets.
	$E_1\subseteq E$ includes the elements $i$ such that the best response of type $i$ to contract $p$ is $a_{i,S}$, for some $S \in \Scal$.
	%
	$E_2\subseteq E$ includes  the elements $i$ such that the best response of type $i$ is $a_{j,S}$ with $j\neq i$ and $S \in \Scal$.
	%
	Finally, $E_3=E \setminus (E_1\cup E_2)$.
	
	We start analyzing the constraint that the best response of types $\theta \in E_1$ impose on the contract.
	Consider a type $\theta=i \in E_1$, and let $a_{i,S}$ be their best response. Notice that $i\in S$.
	%
	Then, from the IC constraint with respect to action $\bar a_{i,S}$ it holds
	
	\[
	p_{\omega_{S}}\frac{1}{10i}\mu + p_{\omega^*}  \frac{1}{5i}\mu+(1-\frac{3}{10i}\mu)p_{\bar\omega}- \frac{1}{20i}\mu \ge  p_{\omega_{S}}\frac{1-\frac{\eta}{2}}{10i} \mu +(1-\frac{1-\frac{\eta}{2}}{10i}\mu)p_{\bar\omega}- \frac{1}{20i} (1-\eta) \mu 
	\]
	implying that
	\[
	p_{\omega_{S}}\ge 1-\frac{4}{\eta}p_{\omega^*}.
	\]
	From this follows that the principal utility against an agent of type $i\in E_1$ is at most
	% \ma{giusto buttare via $\bar \omega$? farà schifo come outcome eh, però magari bisogna dismostrare che $p_{\bar\omega}=0$}
	\begin{align}
	&F_{a_{i,S},\omega_S}(r_{\omega_S}-p_{\omega_S})+F_{a_{i,S},\omega^*}(r_{\omega^*}-p_{\omega^*})+F_{a_{i,S},\bar \omega}(r_{\bar \omega}-p_{\bar\omega})\\
	&\le-\frac{1}{10i}\mu(1-4p_{\omega^*}/\eta)+\frac{1}{5i}\mu(1-p_{\omega^*})\\
	&=\frac{1}{10i}\mu+\frac{1}{5i}p_{\omega^*}\mu(\frac{2}{\eta}-1)
	\end{align}
	
	Now, consider an agent's type $\theta=i\in E_2$, and let $a_{j,S}$, $j \neq i$ be the action played by the agent. 
	Notice that $j \in S$. Then, IC constraint with respect to action $\bar a_{j,S}$ reads
	\[
	p_{\omega_{S}} \frac{1}{10j} \mu + \frac{1}{5j}p_{\omega^*}\mu+(1-\frac{3}{10j}\mu)p_{\bar\omega}- \frac{i}{20j^2}\mu \ge p_{\omega_{S}} \frac{1}{10j} (1-\eta/2) \mu+(1-\frac{1-\frac{\eta}{2}}{10j}\mu)p_{\bar\omega}- \frac{i}{20j^2} (1-\eta) \mu
	\]
	which implies that
	%\[ p_{\omega_{S}} \frac{\eta}{20j} \ge  \frac{i\eta}{20j^2} - \frac{1}{5j} p_{\omega^*} \]
	%and
	\[
	p_{\omega_{S}} \ge \frac{i}{j}- p_{\omega^*} \frac{4}{\eta}. 
	\]
	
	Hence, the principal's expected utility when the realized type is a $\theta=i \in E_2$ is at most:
	\begin{align}
		&F_{a_{j,S},\omega_S}(r_{\omega_S}-p_{\omega_S})+F_{a_{j,S},\omega^*}(r_{\omega^*}-p_{\omega^*})+F_{a_{j,S},\bar \omega}(r_{\bar \omega}-p_{\bar\omega})\\
		&\le-\frac{1}{10j}\mu\left( \frac{i}{j}- p_{\omega^*} \frac{4}{\eta}\right)+\frac{1}{5j}\mu\\
		&=\mu\left(\frac{1}{5j}-\frac{i}{10j^2}+\frac{2}{5j\eta}p_{\omega^*}\right)\\
		&\le\mu\left(\frac{1}{5j}-\frac{i}{10j^2}+\frac{2}{5\eta}p_{\omega^*}\right)
	\end{align}
	
	Now consider the first term $\frac{1}{5j}-\frac{i}{10j^2}$, this is maximized for $j=i-1$ (recall that we cannot have that $j=i$ as $i\in E_2$). To obtain an upper bound on this quantity observe that
	\begin{align}
		\frac{1}{5(i-1)}-\frac{i}{10(i-1)^2}-\frac{1}{10i}&=-\frac{1}{10(i-1)^2i}\\
		&\le -\frac{1}{10(n-1)^2n}\tag{$x\mapsto -\frac{1}{(x-1)^2x}$ is increasing for $x\ge 1$}\\
		&\le-\frac{1}{10n^3}
	\end{align}

	
	
	Hence, the principal's expected utility when the realized type is a $\theta=i \in E_2$ is at most:
	\[
		\mu\left(\frac{1}{10i}-\frac{1}{10n^3}+\frac{2}{5\eta}p_{\omega^*}\right).
	\]
	
	Now consider any type $i\in E_3$. These agents play an action $\bar a_{j, S}$ for some $S$ and $j\in S$ or actions $a^*$ or $a_0$.
	Clearly when actions $\bar a_{j, S}$ and $a_0$ are played the principal utility is at most zero, as the only outcomes reachable from these actions are $\omega_S$ and $\bar\omega$ which have reward $0$. The principal utility is at most zero also for action $a^*$. Indeed consider the IC constraints of action $a^*$ with respect to $a_0$:
	\[
	\sum_{S\in\Scal}F_{a^*,\omega_S}p_{\omega_S}-i\cdot c_{a^*} + F_{a^*,\omega^*} p_{\omega^*}\ge 0
	\]
	which implies that $\epsilon\sum_{S\in\Scal}p_{\omega_S}+(1-m\epsilon)p_{\omega^*}\ge i$. The principal utility, when action $a^*$ is played, is 
	\begin{align}
		\sum_{S\in\Scal} F_{a^*,\omega_S}(r_{\omega_S}-p_{\omega_S})+F_{a^*,\omega^*}(r_{\omega^*}-p_{\omega^*})=&-\epsilon\sum_{S\in\Scal}p_{\omega_S}+(1-m\epsilon)(1-p_{\omega^*})\\
		&\le i-m\epsilon.
	\end{align}
	and thus the principal utility is negative also for action $a^*$.
	
	%\ma{aggiongiere $a_0$ con costo zero che manda determ in $\bar \omega$}. \ma{dici che tutte queste azoni danno utilità negativa ma $a^*$ mi fa fare un sacco di soldi invece... Bisogna far vedere che non la giocano. O meglio che se la giocassero io sto spendendo troppo per fargliela giocare visto che pagano 1 per giocarla. O magari mi sono rincoglionito...}
	
	
	\ma{tbc: } Finally, type $\theta=0$ plays action $a^*$ otherwise the utility is clearly below $\gamma-n^{14}m^{-1}$. Moreover when an agent of type $0$ plays the action $a^*$ the utility of the principal is 
	\[
	-\epsilon\sum_{S\in\Scal}p_{\omega_S}+(1-m\epsilon)(1-p_{\omega^*})
	\]
	
	Define the following set $\bar \Scal:=\{S\in\Scal: p_{\omega_S}\ge1-\frac{4}{\eta}p_{\omega^*}\}$. Combining the upper bounds above on the principal utility we can say that the principal utility is at most
	\[
	\frac{1-\rho}{n}\mu\left[\sum_{i\in E_1}\right(\frac{1}{10i}+\frac{1}{5i}p_{\omega^*}(\frac{2}{\eta}-1)\left)+\sum_{i\in E_2}\left(\frac{1}{10i}-\frac{1}{10n^3}+\frac{2}{5\eta}p_{\omega^*}\right)\right]+\rho(1-m\epsilon)(1-p_{\omega^*})-\epsilon\rho\sum_{S\in\Scal}p_{\omega_S}.
	\]
	Moreover, we can notice that $\sum_{S\in\Scal} p_{\omega_S}\ge |\bar\Scal|(1-\frac{4}{\eta}p_{\omega^*})$, and thus the principal utility is at most an expression in which the coefficient of $p_\omega^*$ is 
	\[
	\frac{1-\rho}{n}\mu\left[\sum_{i\in E_1}\frac{1}{5i}(\frac{2}{\eta}-1)+\sum_{i\in E_2}\frac{2}{5\eta}\right]-\rho(1-m\epsilon)+\frac{4}{\eta}\epsilon\rho|\bar\Scal|.
	\]
	The following calculations shows that this is at most zero:
	\begin{align}
			\frac{1-\rho}{n}\mu&\left[\sum_{i\in E_1}\frac{1}{5i}(\frac{2}{\eta}-1)+\sum_{i\in E_2}\frac{2}{5\eta}\right]-\rho(1-m\epsilon)+\frac{4}{\eta}\epsilon\rho|\bar\Scal|\\
			&\le \frac{1-\rho}{n}\mu\sum_{i\in E_1\cup E_2}\frac{2}{5\eta}-\rho(1-m\epsilon)+4{\rho \epsilon m}{\eta}\\
			&\le \frac{1-\rho}{n}\mu\frac{2}{5\eta}n-\rho(1-m\epsilon)+4\frac{\rho \epsilon m}{\eta}\\
			&=\frac{2}{5\eta}\mu-\rho(1-m\epsilon)+4\frac{\rho \epsilon m}{\eta}\\
			&\le \frac{2}{5}\frac{\mu}{\eta}-\frac{\rho}{2}+4\frac{\rho \epsilon m}{\eta}\\
			&=\frac{2}{5}\frac{n^2}{n^9m}-\frac{1}{2n^6}+4\frac{mn^2}{n^6n^8m}\\
			&=\frac{2}{5}\frac{1}{n^7}-\frac{1}{2n^6}+4\frac{1}{n^{12}}
	\end{align}
	
	which is negative for $n\ge 2$.
	
	Thus any contract with $p_{\omega^*}=0$ achieves larger utility then any contract with $p_{\omega^*}>0$. Thus the principal utility is upper bounded by
	\[
	\frac{1-\rho}{n}\mu\left[\sum_{i\in E_1}\frac{1}{10i}+\sum_{i\in E_2}\left(\frac{1}{10i}-\frac{1}{10n^3}\right)\right]+\rho(1-m\epsilon)-\epsilon\rho|\bar\Scal|.
	\]
	Now observe that 
	\begin{align}
		\frac{1-\rho}{n}\frac{1}{10n^3}&\ge \frac{\mu}{20n^4}\\
		&=\frac{1}{20n^13m}\\
		&=\frac{1}{n^14m}\tag{$n\ge O(1)$}\\
		&=\rho\epsilon
	\end{align}
	
	and thus we can find that the principal utility is upper bounded by
	\[
	\frac{1-\rho}{n}\mu\sum_{i\in E}\frac{1}{10i}+\rho(1-m\epsilon)-\epsilon\rho(|\bar\Scal|+|E\setminus E_1|).
	\]
	Now we complete the set $\bar S$ to make it a set cover of $E$ in the following way. For each element $v$ of $E\setminus E_1$ we pick a set $s(v)\in\Scal$ such that $v\in s(v)$ and we claim that $\Scal^*:=\bar\Scal\cup( \cup_{v\in E\setminus E_1}s(v))$ is a cover of $E$, since by construction the set $\bar S$ is a cover of $E_1$ and $\cup_{v\in E\setminus E_1}s(v)$ is a cover of $E\setminus E_1$. Thus $\Scal^*$ is a cover of $E$ and thus has size at least $k+1$, also note that $|\cup_{v\in E\setminus E_1}s(v)|\le |E\setminus E_1|$. The proof is concluded by observing that $|\bar \Scal|+|E\setminus E_1|\ge |\Scal^*|\ge k+1$ and thus the principal utility is upper bounded by
	\[
	\frac{1-\rho}{n}\mu\sum_{i\in E}\frac{1}{10i}+\rho(1-m\epsilon)-\epsilon\rho(k+1)=\gamma-\epsilon\rho=\gamma-\frac{1}{n^{14}m}.
	\]
	
%	\ma{==================OLD==================}
%	\[ 
%	\frac{1}{5j} - \frac{i}{10j^2} +  \frac{1}{10j} p_{\omega^*} \frac{4}{\eta}
%	\le \frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*}  
%	\]
%	\mat{da dimostrare, o checkato su wolfram}
%	
%	Finally, consider the set of agent types $\theta=i\in E_3$. These agent's plays or an action $\bar a_{j,S}$, $j\in E$, $S\in \Scal$, or action $a^*$, or \mat{or void action (aggiungere al modello)}. It is easy to see that the principal's utility is at most $0$ for all these possible actions. \ma{qui vedo un problemino}
%	
%	Finally, type $\theta=0$ plays action $a^*$ otherwise the utility is clearly below $\gamma-n^{14}m^{-1}$.
%
%
%
%Let $\bar \Scal$ be the sets $S$ such that $p_{\omega_S}\ge 1- 4 p_{\omega^*}$.
%Then, the principal's utility is at most 
%\[ \frac{1-\rho}{n} \ell \left[\sum_{i \in E_1}( \frac{1}{5i} (1-p_{\omega^{*}}) - \frac{1}{10i}( 1-4p_{\omega^*}/\eta))  + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*})\right] + \rho (1-m\epsilon) (1-p_{\omega^*}) - \rho \epsilon |\bar\Scal|(1-4p_{\omega^*}/\eta)\]
%\[\le \frac{1-\rho}{n} \ell \left[\sum_{i \in E_1}( \frac{1}{5i}  - \frac{1}{10i}( 1-4p_{\omega^*}/\eta))  + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*})\right] + \rho (1-m\epsilon) (1-p_{\omega^*}) - \rho \epsilon |\bar\Scal|(1-4p_{\omega^*}/\eta)   \]
%
%
%Then, since
%\[\frac{1-\rho}{n} \ell  n \frac{2}{5} \frac{1}{\eta} - \rho (1-m\epsilon) + 4 \rho \epsilon m \frac{1}{\eta} \le  \ell/\eta -\rho/2 + 4 \rho \epsilon m/\eta=n^{-7}m^{-1} - n^{-6}/2 + 4 n^{-12}<0 \]
%for $n$ large enough, it is the case that
%
%\[\arg \max_{p_{\omega^*}}  \frac{1-\rho}{n} \ell [\sum_{i \in V^*}( \frac{1}{5i}  - \frac{1}{10i}( 1-4p_{\omega^*}/\eta))  + \sum_{i \notin V^*} (\frac{1}{10i}-\frac{1}{40n^3}  + \frac{2}{5j\eta}p_{\omega^*})] + \rho (1-m\epsilon) (1-p_{\omega^*}) - \rho \epsilon |\bar\Scal|(1-4p_{\omega^*}/\eta)= 0,\]
%
%Hence, setting $p_{\omega^*}=0$ the principal's utility is at most
%\begin{align}
%	&\frac{1-\rho}{n} \ell \left[\sum_{i \in E_1}( \frac{1}{5i}  - \frac{1}{10i})  + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}) \right] + \rho (1-m\epsilon) - \rho \epsilon |\bar\Scal|\\
%	&=\frac{1-\rho}{n} \ell \left[\sum_{i \in E_1} \frac{1}{10i} + \sum_{i \in E \setminus E_1} (\frac{1}{10i}-\frac{1}{40n^3}) \right] + \rho (1-m\epsilon) - \rho \epsilon |\bar\Scal|\\
%	& \le \frac{1-\rho}{n} \ell \sum_{i \in E} \frac{1}{10i}    + \rho (1-m\epsilon) - \rho \epsilon (|\bar\Scal|+ |E\setminus E_1|) 
%\end{align}
%where the last inequality follows since 
%\[\frac{1-\rho}{n} \ell \frac{1}{40n^3}\ge n^{-13} m^{-1}/80 \ge n^{-14} m^{-1}  = \rho \epsilon. \]
%for $n$ large enough.
%
%Let define the function $s:E\rightarrow\Scal$ that assign to each element $i \in E$ a set $S \in \Scal$ such that $i\in S$.
%Now, notice that there exists a set cover of size $|\bar\Scal|+ |E\setminus E_1|$ taking the set $S=\bar\Scal\cup (\cup_{v \in V\setminus V^*} s(v))$. Indeed, all the elements in $E_1$ are covered by a set in $\Scal$ by definition, while $\cup_{E \in E \setminus E_1} s(v)$ clearly covers all the elements not in $E_1$.
%
%Thus,the principal's utility is at most
%\[ \frac{1-\rho}{n} \ell \sum_{i \in V} \frac{1}{10i}    + \rho (1-m\epsilon) - \rho \epsilon (k+1)\le \gamma - \rho \epsilon= \gamma- n^{-14} m^{-1}, \]
%concluding the proof.
%
%
%
%

\end{proof}

==> src/multiplicative.tex <==
\section{multiplicative}
\mat{qui è thrash! open question se si può fare approssimazione meglio che numero di tipi per distribuzioni uniformi (o equivalentemente "polynomially balanced")}
it would be interesting to find properties such that a constant or better multiplicative approximation is possible.
For instance "Bayesian analysis of linear contracts" provides some assumption to guarantee a constant factor approximation.

Let assume that the partition is balanced, i.e., for each types $\theta_1$ and $\theta_2$, it holds $\mu_{\theta_1}/\mu_{\theta_2}\le M$.

Take $\theta_1\le \theta_2$ and assume that 
\[ F_{a_1} (r-p^1) \ge F_{a_2} (r-p^2).\]

Now consider the agent $\theta_1$ with payment $p^2 \theta_1/\theta_2$.
It incentivizes $a_2$ and provides utility

\[F_{a_2} (r-p^2 \theta_1/\theta_2)\ge F_{a_2} r(1-\theta_1/\theta_2)\ge F_{a_2} r/2 \]

Hence, 
\[ F_{a_2} r/2 \le M F_{a_2} (r-p^2) \]
and
\[F_{a_2} p^2 \le 	\frac{M-1}{M} F_{a_2} r/2  \]

\subsection{linear contract inspired}

Partition the types in intervals $\Theta_i=[2^{-i-1},2^{-i}]$.

Let $p_i= \max_p F_{a(p,2^{-i})} (r-p)$. 

Then, 
\[F_{a(p_i,2^{-i})} (r-p_i)\le 2^{-j+ i} _{a(p_i,2^{-i})} (r-p_i) \]


Then,
\[ \sum_i \gamma_i F_{a(p_i,2^{-i})} (r-p_i) \le   \]


==> src/prelims_menu_rand.tex <==
\subsection{Menus of Randomized Contracts}\label{sec:preliminaries_contracts}

\mat{non modificato da qua. Copiato da un altro paper solo per avere un po di notazione}

We study Bayesian principal-agent problems in which there is an additional \emph{type-reporting} stage in which the principal proposes to the agent a menu of randomized contracts to choose from.

A \emph{randomized contract} is a probability distribution $\gamma$ over $\mathbb{R}^m_+$, \emph{i.e.}, over the set of vectors $p \in \mathbb{R}^m_+$ representing all the possible contracts.
% defined by a payment $p_\omega \geq 0$ for each outcome $\omega \in \Omega$.
%
We use $p \sim \gamma$ to denote that the (random) contract $p$ is distributed according to $\gamma$, and write $\mathbb{E}_{p \sim \gamma} [\cdot]$ to indicate the expectation taken with respect to the randomness of $p$.
%
We denote by $\supp (\gamma)$ the support of $\gamma$.
%
When $\gamma$ has a finite support, \emph{i.e.}, $|\supp (\gamma)| < \infty$, we let $\gamma_p $ be the probability that $\gamma$ assigns to contract $p \in \mathbb{R}^m_+$.


A \emph{menu of randomized contracts} is defined by a tuple $\Gamma = \left( \gamma^\theta \right)_{\theta \in \Theta}$ specifying a probability distribution $\gamma^\theta$ over $\mathbb{R}^m_+$ for each agent's type $\theta \in \Theta$.


The interaction between the principal and an agent of type $\theta \in \Theta$ goes as follows:
%
\begin{itemize}
	\item[(i)] the principal publicly commits to a menu $\Gamma = \left( \gamma^\theta \right)_{\theta \in \Theta}$ of randomized contracts;
	%
	\item[(ii)] the agent reports a type $\hat \theta \in \Theta$ to the principal, possibly different from the true type $\theta$;
	% so as to maximize their expected utility $\mathbb{E}_{p \sim \gamma^{\theta'}} \left[ \sum_{\omega \in \Omega} F_{\theta, b^\theta(p), \omega} \, p_\omega - c_{\theta, b^\theta(p)}   \right]$.
	%
	\item[(iii)] the principal draws a contract $p \sim \gamma^{\hat \theta}$ and communicates it to the agent;
	%
	\item[(iv)] the agent plays the best-response action $b^\theta(p)$.
\end{itemize}



The goal of the principal is to commit to a utility-maximizing menu of randomized contracts, selecting among those that are \emph{dominant-strategy incentive compatible} (DSIC).\footnote{Notice that, by a revelation-principle-style argument (see the book by~\citet{shoham2008multiagent} for some examples of these kind of arguments), focusing on DSIC menus of contracts is w.l.o.g. when looking for a principal-optimal menu.}
%
Formally, a menu $\Gamma = \left( \gamma^\theta \right)_{\theta \in \Theta}$ of randomized contracts is DSIC if the following holds:
\begin{equation}\label{eq:dsic}
	\mathbb{E}_{p \sim \gamma^\theta} \left[  \sum_{\omega \in \Omega} F_{\theta, b^\theta(p), \omega} \, p_\omega - c_{\theta, b^\theta(p)} \right]  \geq \mathbb{E}_{p \sim \gamma^{\hat \theta}} \left[  \sum_{\omega \in \Omega} F_{\theta, b^\theta(p),\omega} \, p_\omega - c_{\theta, b^\theta(p)}  \right]    \forall \hat \theta \neq \theta \in \Theta.
\end{equation}
%
Intuitively, the conditions above guarantee that the expected utility of an agent of type $\theta \in \Theta$ under the randomized contract $\gamma^\theta$ is greater than or equal to that obtained under $\gamma^{\hat \theta}$, for any $\hat \theta \neq \theta \in \Theta$.
%
This ensures that the agent is always better off reporting their true type to the principal.
%
Then, the principal's goal is to find a menu $\Gamma = \left( \gamma^\theta \right)_{\theta \in \Theta}$ that is optimal for the following problem:
\begin{equation}\label{eq:problem}
	\max_{\Gamma = \left( \gamma^\theta \right)_{\theta \in \Theta}} \quad \sum_{\theta \in \Theta} \mu_\theta \, \mathbb{E}_{p \sim \gamma^\theta} \left[  \sum_{\omega \in \Omega} F_{\theta, b^\theta(p), \omega} \, r_\omega -\sum_{\omega \in \Omega} F_{\theta, b^\theta(p), \omega} \, p_\omega \right] \quad \textnormal{s.t.} \quad \textnormal{Equation~\eqref{eq:dsic}},
\end{equation}
%
whose objective is the principal's expected utility for a DSIC menu of randomized contracts.


We also consider the case, already investigated by~\citet{guruganesh2021contracts}, in which the menu of contracts is made by non-randomized contracts.
%
Formally, we denote a \emph{menu of deterministic contracts} by a tuple $P = \left(  p^\theta \right)_{\theta \in \Theta}$, containing a contract $p^\theta \in \mathbb{R}^m_+$ for each agent's type $\theta \in \Theta$.
%
In this case, the principal does \emph{not} draw a contract in step (iii) of the interaction, but they simply adopt contract $p^{\hat \theta}$, where $\hat \theta \in \Theta$ is the type reported by the agent.
%
Thus, all the definitions above can be specialized to the case of menus of deterministic contracts by dropping expectations. 
